Publicly-Verifiable Deletion via Target-Collapsing Functions

We build quantum cryptosystems that support publicly-verifiable deletion from standard cryptographic assumptions. We introduce target-collapsing as a weakening of collapsing for hash functions, analogous to how second preimage resistance weakens collision resistance; that is, target-collapsing requires indistinguishability between superpositions and mixtures of preimages of an honestly sampled image. We show that target-collapsing hashes enable publicly-verifiable deletion (PVD), proving conjectures from [Poremba, ITCS'23] and demonstrating that the Dual-Regev encryption (and corresponding fully homomorphic encryption) schemes support PVD under the LWE assumption. We further build on this framework to obtain a variety of primitives supporting publicly-verifiable deletion from weak cryptographic assumptions, including: - Commitments with PVD assuming the existence of injective one-way functions, or more generally, almost-regular one-way functions. Along the way, we demonstrate that (variants of) target-collapsing hashes can be built from almost-regular one-way functions. - Public-key encryption with PVD assuming trapdoored variants of injective (or almost-regular) one-way functions. We also demonstrate that the encryption scheme of [Hhan, Morimae, and Yamakawa, Eurocrypt'23] based on pseudorandom group actions has PVD. - $X$ with PVD for $X \in \{$attribute-based encryption, quantum fully-homomorphic encryption, witness encryption, time-revocable encryption$\}$, assuming $X$ and trapdoored variants of injective (or almost-regular) one-way functions.

==> OWF.tex <==
\section{OWF-based certified deletion}

Let $f = \{f_\secp : \{0,1\}^{m(\secp)} \to \{0,1\}^{n(\secp)}\}_{\secp \in \bbN}$ be a regular (\james{hopefully we can relax the regularity requirement somewhat}) one-way function and let $\cA = \{\cA_\secp\}_{\secp \in \bbN}$ be any QPT adversary. \alex{How is regularity defined here? Is it a similar definition as in Mark Zhandry's paper on collapsing hashes?}\james{For now I mean exactly regular, so each element of the image has the same number of preimages. But we can try to relax to either Mark's definition of semi-regularity, or perhaps almost-regularity (the relative size of each set of preimages is within a fixed polynomial ratio).}\james{An additional property we may need is that the range of the OWF (as a subset of the codomain) is somehow efficiently describable, so we can restrict the linear map to be only applied to elements in the range. Otherwise, it may be the case that for many pairs of vectors in the domain of the linear map, only 0 or 1 of them are valid images of the OWF. But maybe this can be generically obtained by compressing the image with a universal hash function.  }

Consider the following experiment $\Exp_{f,\cA,\secp}(b)$.

\begin{enumerate}
    \item The challenger samples a uniformly random full rank linear map $h: \bbF_2^{n} \to \bbF_2^{n-1}$ and prepares the state
    \[\frac{1}{\sqrt{2^m}}\sum_{x \in \{0,1\}^m}(-1)^{b \cdot p_{f,h}(x)}\ket{x}_X\ket{h(f(x))}_Z,\]
    where $p_{f,h}(x) = 0$ iff, letting $y \coloneqq f(x) \in \{0,1\}^n, z \coloneqq h(y) \in \{0,1\}^{n-1}$, it holds that $y$ is the lexicographially first string such that $h(y) = z$. The challenger then measures the $Z$ register in the standard basis to obtain $z$, and the remaining state collapses to 
    \[\frac{1}{\sqrt{2^{m-n+1}}}\left(\sum_{x : f(x) = y_{z,0}}\ket{x}_X + (-1)^b\sum_{x : f(x) = y_{z,1}}\ket{x}_X\right),\] where $y_{z,0},y_{z,1} \in \{0,1\}^n$ are the two strings such that $h(y_{z,0}) = h(y_{z,1}) = z$, ordered lexicographically.
    \item The challenger sends $h,z$, and the $X$ register to $\cA_\secp$, who outputs a classical deletion certificate $\pi$ and a left-over quantum state $\rho$.
    \item If $h(f(\pi)) = z$, output $\rho$, and otherwise output $\bot$.
\end{enumerate}

\begin{theorem}
\[\TD\left(\Exp_{f,\cA,\secp}(0),\Exp_{f,\cA,\secp}(1)\right) = \negl(\secp).\]
\end{theorem}

\begin{proof}
\james{Sketch} The proof will basically follow the same strategy used above in the collapsing-based certified deletion game.
\begin{enumerate}
	\item Hybrid 1: Entangle the phase bit with a challenger's register $C$ and measure this register at the end of experiment to obtain $b$.
	\item Hybrid 2: If the adversary outputs a valid deletion certificate $\pi$, project register $C$ onto $\frac{1}{\sqrt{2}}\left(\ket{0} + (-1)^{p_{f,h}(\pi)}\ket{1}\right).$ In this hybrid, $b$ is then a uniformly random bit.
\end{enumerate}
To show indistinguishability between Hybrid 1 and 2, we need to define an experiment where the bit $p_{f,h}(x)$ is measured on register $X$ before the state is given to the adversary. Let \[\ket{0_{f,h,z}} \coloneqq \frac{1}{\sqrt{2^{m-n}}}\sum_{x:f(x)=y_{z,0}}\ket{x}, ~~ \ket{1_{f,h,z}} \coloneqq \frac{1}{\sqrt{2^{m-n}}}\sum_{x:f(x)=y_{z,1}}\ket{x},\] and $\ket{+_{f,h,z}} \coloneqq \frac{1}{\sqrt{2}}(\ket{0_{f,h,z}} + \ket{1_{f,h,z}}), \ket{-_{f,h,z}} \coloneqq \frac{1}{\sqrt{2}}(\ket{0_{f,h,z}} - \ket{1_{f,h,z}})$. Then, measuring this bit on register $X$ collapses the state as follows: \[\frac{1}{\sqrt{2}}\ket{0}_C\ket{+_{f,h,z}}_X + \frac{1}{\sqrt{2}}\ket{1}_C\ket{-_{f,h,z}}_X \to \frac{1}{2}\ket{+}\bra{+}_C \otimes \ket{0_{f,h,z}}\bra{0_{f,h,z}}_X + \frac{1}{2}\ket{-}\bra{-}_C \otimes \ket{1_{f,h,z}}\bra{1_{f,h,z}}_X\] 
	
	
By [AAS, HMY] and the fact that all $\ket{+_{f,h,z}}$ and $\ket{-_{f,h,z}}$ (for all $h,z$) are orthogonal states, which follows from the regularity of $f$, any $\cA$ that can distinguish this switch can be used to map the state $\ket{0_{f,h,z}} \to \ket{1_{f,h,z}}$ (on average over $h,z$). This is impossible due to the one-wayness of $f$ and the fact that $f$ is regular (which allows the reduction to go through). Moreover, in this experiment, there is a negligible probability that the adversary outputs a valid $\pi$ but projecting register $C$ onto $\frac{1}{\sqrt{2}}\left(\ket{0} + (-1)^{p_{f,h}(\pi)}\ket{1}\right)$ fails, which again follows from the one-wayness and regularity of $f$. Thus, adding this projection to Hybrid 2 must only have a negligible affect on the experiment.

\end{proof}

\paragraph{Applications}
\begin{itemize}
    \item By purifying, this theorem can be used to obtain bit commitments with publicly-verifiable certified deletion. This will imply ZK proofs with publicly-verifiable everlasting zero-knowledge, and secure computation with publicly-verifiable EST.
    \item If $f$ admits a trapdoor that allows to prepare the uniform superposition over preimages for any image (a special case of this is the standard notion of an injective trapdoor function), then this implies public-key encryption with publicly-verifiable certified deletion.
\end{itemize}

==> applications.tex <==
\section{Publicly-Verifiable Certified Deletion from Almost Regular One-Way Functions}

\subsection{Definitions}

A \emph{canonical quantum bit commitment} consists of a family of pairs of unitaries $\{(Q_{\secp,0},Q_{\secp,1})\}_{\secp \in \bbN}$. To commit to a bit $b$, the committer applies $Q_{\secp,b}$ to the all-zeros state $\ket{0}$ to obtain a state on registers $C$ and $R$, and sends register $C$ to the receiver. To open, the committer sends the bit $b$ and the remaining state on register $R$. The receiver applies $Q_{\secp,b}^\dagger$ to registers $(C,R)$, measures the result in the standard basis, and accepts if all zeros are observed.

\begin{definition}[Computational Hiding]
A canonical quantum bit commitment $\{(Q_{\secp,0},Q_{\secp,1})\}_{\secp \in \bbN}$ satisfies \emph{computational hiding} if for any QPT adversary $\{\cA_\secp\}_{\secp \in \bbN}$,

\[\left|\Pr\left[\cA_\secp(\Tr_R\left(Q_{\secp,0}\ket{0}\right)) = 1\right] - \Pr\left[\cA_\secp(\Tr_R\left(Q_{\secp,1}\ket{0}\right)) = 1\right] \right| = \negl(\secp).\]
\end{definition}

\begin{definition}[Honest Binding]
A canonical quantum bit commitment $\{(Q_{\secp,0},Q_{\secp,1})\}_{\secp \in \bbN}$ satisfies \emph{honest binding} if for any auxiliary family of states $\{\ket{\psi_\secp}\}_{\secp \in \bbN}$ on register $Z$ and any family of physically realizable unitaries $\{U_\secp\}_{\secp \in \bbN}$ on registers $R,Z$, 

\[\left\| \left(Q_{\secp,1}\dyad{0}{0}Q_{\secp,1}^\dagger\right)U\left(Q_{\secp,0}\ket{0}\ket{\psi}\right)\right\| = \negl(\secp).\]
\end{definition}

\begin{definition}[Publicly-Verifiable Certified Everlasting Hiding]
A canonical quantum bit commitment $\{(Q_{\secp,0},Q_{\secp,1})\}_{\secp \in \bbN}$ satisfies \emph{publicly-verifiable certified everlasting hiding} if there exists a measurement $\{V_{\secp}\}_{\secp \in \bbN}$ on register $R$, a measurement $\{D_{\secp}\}_{\secp \in \bbN}$ on register $C$, and a classical predicate $\Ver(\cdot,\cdot) \to \{\top,\bot\}$ that satisfy the following properties.

\begin{itemize}
    \item \textbf{Correctness of deletion.} For any $b \in \{0,1\}$, it holds that
    \[\Pr\left[\Ver(\vk,\pi) = \top : (\vk,\pi) \gets (V_\secp \otimes D_\secp)Q_{\secp,b}\ket{0}\right] = 1-\negl(\secp).\]
    \item \textbf{Certified everlasting hiding.} For any two-part adversary $\cA = (\cA_{\secp,1},\cA_{\secp,2})_{\secp \in \bbN}$ where $\{\cA_{\secp,1}\}_{\secp \in \bbN}$ is QPT and $\{\cA_{\secp,2}\}_{\secp \in \bbN}$ is unbounded, it holds that 
    \[\left|\Pr\left[\mathsf{EvExp}_{\cA}(\secp,0) = 1\right] - \Pr\left[\mathsf{EvExp}_{\cA}(\secp,1) = 1\right]\right| = \negl(\secp),\] where $\mathsf{EvExp}_{\cA}(\secp,b)$ is the following experiment.
    \begin{itemize}
        \item Prepare $Q_{\secp,b}\ket{0}$, measure register $R$ with $V_\secp$ to obtain $\vk$, and send $(\vk,C)$ to $\cA_{\secp,1}$.
        \item Parse $\cA_{\secp,1}$'s output as a deletion certificate $\pi$ and a left-over state $\rho$. If $\Ver(\vk,\pi) = \bot$, output $\bot$ and abort the experiment.
        \item Run $\cA_{\secp,2}$ on input $\rho$ until it outputs a bit.
    \end{itemize}
\end{itemize}
\end{definition}

\james{Define public-key encryption with certified deletion (for section above too)}

\james{Define zero-knowledge proof with certified everlasting zero-knowledge}


%\subsection{Constructions}

%Let $\{H_\secp : \{0,1\}^{4\secp} \to \{0,1\}^\secp\}_{\secp \in \bbN}$ be a family of targeted-collapsing and targeted-collision-resistant hash functions (which, by our main theorem, implies certified everlasting targeted-collapsing). We define a quantum canonical bit commitment with publicly-verifiable certified everlasting hiding as follows.

%\begin{itemize}
    %\item $Q_{\secp,b}$ is the unitary that prepares the state
    %\[\frac{1}{\sqrt{|H_\secp|} \cdot 2^{4\secp}}\sum_{h \in H_\secp,r,x \in \{0,1\}^{4\secp},}(-1)^{b \cdot (x \cdot r)}\ket{h,r,h(x)}_R\ket{h,r,x,h(x)}_C.\]
    %\item $V_\secp$ measures the first and third parts of $R$ in the standard basis to obtain $\vk = (h,y)$, and $D_\secp$ measures the third part of $C$ in the standard basis to obtain $\pi = x$.
    %\item $\Ver((h,y),x)$ outputs $\top$ iff $h(x) = y$.
%\end{itemize}

%\begin{theorem}
%The above construction satisfies computational hiding, honest binding, and publicly-verifiable certified everlasting hiding.
%\end{theorem}

%\begin{proof}
%\begin{itemize}
    %\item \james{computational hiding is straightforward from targeted-collapsing}
    %\item \james{to show honest binding, we can establish that the fidelity between the states on register $C$ when $b = 0$ vs $b=1$ is negligible, which will follow from a standard Chebyshev argument}
    %\item \james{certified everlasting hiding is straightforward from certified everlasting targeted-collapsing}
%\end{itemize}
%\end{proof}

%\james{Prior work will give the implication to zero-knowledge proofs for NP with publicly-verifiable certified everlasting zero-knowledge}



%\begin{itemize}
    %\item Certified everlasting target-collapsing function with exponential compression implies commitments with publicly-verifiable certifiable deletion (which imply zero-knowledge with publicly-verifiable certified deletion and secure computation with publicly-verifiable everlasting security transfer). Thus, these primitives all follow from injective one-way functions.
    %\item Trapdoor certified everlasting target-collapsing function implies PKE with publicly-verifiable certified deletion. Thus, this follows from injective trapdoor functions.
%\end{itemize}

==> defs.tex <==
\section{Definitions: Target-Collapsing and Target-Collision-Resistance}

Unruh~\cite{cryptoeprint:2015/361} introduced the notion of collapsing hash functions in his seminal work on computationally binding quantum commitments. This property is captured by the following definition.

\begin{definition}[Collapsing Hash Function \cite{cryptoeprint:2015/361}] A hash function family $\algo H = \{H_\lambda\}_{\lambda \in \N}$ is called collapsing if, for every $\QPT$ adversary $\algo A$,
$$
|
\Pr[ \mathsf{CollapseExp}_{\algo H,\algo A,\lambda}(0)=1] - \Pr[ \mathsf{CollapseExp}_{\algo H,\algo A,\lambda}(1)=1]
| \leq \negl(\lambda).
$$
Here, the experiment $\mathsf{CollapseExp}_{\algo H,\algo A,\lambda}(b)$ is defined as follows:
\begin{enumerate}
    \item The challenger samples a random hash function $h \rand H_\lambda$, and sends a description of $h$ to $\algo A$.
    \item $\algo A$ responds with a (classical) string $y \in \bit^{n(\lambda)}$ and $m(\lambda)$-qubit quantum state in system $X$.
    \item The challenger coherently computes $h$ (into an auxiliary system $Y$) given the state in system $X$, and then performs a two-outcome measurement on $Y$ indicating whether the output of $h$ equals $y$. If $h$ does not equal $y$ the challenger aborts and
outputs $\bot$.

\item If $b=0$, the challenger does nothing. Else, if $b=1$, the challenger measures the $m(\lambda)$-qubit system $X$ in the computational basis. The challenger returns the state in system $X$ to $\algo A$.

\item $\algo A$ returns a bit $b'$, which we define as the output of the experiment.
\end{enumerate}
\end{definition}


==> dual-regev.tex <==
\section{Publicly-Verifiable Deletion from Dual-Regev Encryption}\label{sec:Dual-Regev}

In this section, we recall the constructions of Dual-Regev public-key encryption as well as fully homomorphic encryption with publicly-verifiable deletion introduced by Poremba~\cite{Poremba22}. Using our main result on certified-everlasting target-collapsing hashes in \Cref{thm:CETC-generalization}, we prove the \emph{strong Gaussian-collapsing conjecture} in~\cite{Poremba22}, and then conclude that the aforementioned constructions achieve certified-everlasting security assuming the quantum hardness of $\LWE$ and $\SIS$.

First, let us recall the definition of public-key encryption with publicly-verifiable deletion. 

\subsection{Definition: Encryption with Publicly-Verifiable Deletion}

A public-key encryption (PKE) scheme with publicly-verifiable deletion (PVD) has the following syntax.

\begin{itemize}
    \item $\KeyGen(1^\secp) \to (\pk,\sk)$: the key generation algorithm takes as input the security parameter $\secp$ and outputs a public key $\pk$ and secret key $\sk$.
    \item $\Enc(\pk,m) \to (\vk,\ket{\ct})$: the encryption algorithm takes as input the public key $\pk$ and a plaintext $m$, and outputs a (public) verification key $\vk$ and a ciphertext $\ket{\ct}$.
    \item $\Dec(\sk,\ket{\ct}) \to m$: the decryption algorithm takes as input the secret key $\sk$ and a ciphertext $\ket{\ct}$ and outputs a plaintext $m$.
    \item $\Del(\ket{\ct}) \to \pi$: the deletion algorithm takes as input a ciphertext $\ket{\ct}$ and outputs a deletion certificate $\pi$.
    \item $\Vrfy(\vk,\pi) \to \{\top,\bot\}$: the verify algorithm takes as input a (public) verification key $\vk$ and a proof $\pi$, and outputs $\top$ or $\bot$.
\end{itemize}

\begin{definition}[Correctness of deletion]\label{def:correctness-deletion}
A PKE scheme with PVD satisfies \emph{correctness of deletion} if for any $m$, it holds with $1-\negl(\secp)$ probability over $(\pk,\sk) \gets \Gen(1^\secp), (\vk,\ket{\ct}) \gets \Enc(\pk,m),\pi \gets \Del(\ket{\ct}),\mu \gets \Vrfy(\vk,\pi)$ that $\mu = \top$.
\end{definition}

\begin{definition}[Certified deletion security]\label{def:security-deletion}
A PKE scheme with PVD satisfies \emph{certified deletion security} if it satisfies standard semantic security, and moreover, for any QPT adversary $\{\cA_\secp\}_{\secp \in \bbN}$, it holds that 
\[\TD\left(\mathsf{EvPKE}_{\cA,\secp}(0),\mathsf{EvPKE}_{\cA,\secp}(1)\right) = \negl(\secp),\] where the experiment $\mathsf{EvPKE}_{\cA,\secp}(b)$ is defined as follows.
\begin{itemize}
    \item Sample $(\pk,\sk) \gets \Gen(1^\secp)$ and $(\vk,\ket{\ct}) \gets \Enc(\pk,b)$.
    \item Run $\cA_\secp(\pk,\vk,\ket{\ct})$, and parse their output as a deletion certificate $\pi$ and a left-over quantum state $\rho$.
    \item If $\Vrfy(\vk,\pi) = \top$, output $\rho$, and otherwise output $\bot$.
\end{itemize}
\end{definition}

\ \\
Before we introduce the
Dual-Regev public-key schemes proposed by Poremba~\cite{Poremba22}, let us first recall some basic facts about
Gaussian superpositions.

\subsection{Gaussian 
Superpositions}

Given a modulus $q \in \N$, and integer $m \in \N$ and a parameter $\sigma \in (\sqrt{2m},q/\sqrt{2m})$, we consider
Gaussian superposition states over the finite set $\Z^m \cap (-\frac{q}{2},\frac{q}{2}]^m$ of the form
    $$
 \ket{\psi} =    \sum_{\vec x \in \Z_q^m} \rho_\sigma(\vec x) \ket{\vec x}.
    $$
The state $\ket{\psi}$ is not normalized for convenience. A standard tail bound~\cite[Lemma 1.5 (ii)]{Banaszczyk1993} implies that (the normalized variant of) $\ket{\psi}$ is within negligible trace distance of a \emph{truncated} discrete Gaussian superposition $ \ket{\tilde{\psi}}$
with support $\{\vec x \in \Z_q^m : \|\vec x\| \leq \sigma \sqrt{\frac{m}{2}}\}$, where
$$
\ket{\tilde{\psi}}
= 
\left(\sum_{\vec z \in \Z_q^m,\|\vec z\| \leq \sigma \sqrt{\frac{m}{2}} } \rho_{\frac{\sigma}{\sqrt{2}}}(\vec z) \right)^{-\frac{1}{2}}\sum_{\vec x \in \Z_q^m : \|\vec x\| \leq \sigma \sqrt{\frac{m}{2}}}
\rho_\sigma(\vec x) \ket{\vec x}.
$$
Note that a measurement of $\ket{\tilde{\psi}}$ results in a sample from the truncated discrete Gaussian distribution $D_{\Z_q^m,\frac{\sigma}{\sqrt{2}}}$.
We remark that Gaussian superpositions with parameter $\sigma = \Omega(\sqrt{m})$ can be efficiently implemented using standard quantum state preparation techniques; for example using \emph{quantum rejection sampling} and the \emph{Grover-Rudolph algorithm}~\cite{Grover2002CreatingST,Regev05,Brakerski18,brakerski2021cryptographic}.

Let $\vec A \in \Z_q^{n \times m}$ be a matrix. We use the following algorithm, denoted by $\mathsf{GenGauss}(\vec A,\sigma)$ which prepares a partially measured Gaussian superposition of pre-images of a randomly generated image.
\begin{enumerate}
\item Prepare a Gaussian superposition in system $X$ with parameter $\sigma > 0$:
    $$
 \ket{\psi} =    \sum_{\vec x \in \Z_q^m} \rho_\sigma(\vec x) \ket{\vec x} \otimes \ket{\vec 0}.
    $$
\item Apply the unitary $U_{\vec A}: \ket{\vec x}\ket{\vec 0} \rightarrow \ket{\vec x} \ket{\vec A \cdot \vec x \Mod{q}}$, which results in the state
$$
 \ket{ \psi} =   \sum_{\vec x \in \Z_q^m} \rho_\sigma(\vec x) \ket{\vec x} \otimes \ket{\vec A \cdot \vec x \Mod{q}}.
  $$
  \item Measure the second register in the computational basis, which results in $\vec y \in \Z_q^n$ and a state
    $$
    \ket{\psi_{\vec y}} = \sum_{\substack{\vec x \in \Z_q^m:\\ \vec A \vec x= \vec y \Mod{q}}} \rho_\sigma(\vec x) \ket{\vec x}.
    $$
\end{enumerate}

Finally, we use the following lemma which characterizes the Fourier transform of a partially measured Gaussian superposition.

\begin{lemma}[\cite{Poremba22}, Lemma 16]\label{lem:duality}
Let $m \in \N$, $q \geq 2$ be a prime and $\sigma \in (\sqrt{2m},q/\sqrt{2m})$.
Let $\vec A \in \Z_q^{n \times m}$ be a matrix whose columns generate $\Z_q^n$ and let $\vec y \in \Z_q^n$ be arbitrary. Then, the $q$-ary quantum Fourier transform of the (normalized variant of the) Gaussian coset state
$$
 \ket{\psi_{\vec y}} = \sum_{\substack{\vec x \in \Z_q^m\\ \vec A \vec x = \vec y \Mod{q}}}\rho_{\sigma}(\vec x) \ket{\vec x}
$$
is within negligible (in $m \in \N$) trace distance of the (normalized variant of the) Gaussian state
$$
 \ket{\hat\psi_{\vec y}} = \sum_{\vec s \in \Z_q^n} \sum_{\vec e \in \Z_q^m} \rho_{q/\sigma}(\vec e) \, \omega_q^{-\langle\vec s,\vec y \rangle} \ket{\vec s^\intercal \vec A + \vec e^\intercal \Mod{q}}.
$$
\end{lemma}


\subsection{(Strong) Gaussian-Collapsing Property.}

We use the following result which says that the Ajtai hash function is target-collapsing with respect to the truncated discrete Gaussian distribution.

\begin{theorem}[Gaussian-collapsing property, \cite{Poremba22}, Theorem 4]\label{thm:Gauss-collapsing}
Let $n\in \N$ and $q$ be a prime with $m \geq 2n \log q$, each parameterized by $\lambda \in \N$. Let  $\sigma \in (\sqrt{2m},q/\sqrt{2m})$.
Then,
the following samples are computationallyindistinguishable assuming the quantum hardness of decisional $\mathsf{LWE}_{n,q,\alpha q}^m$, for any noise ratio $\alpha \in (0,1)$ with relative noise magnitude $1/\alpha= \sigma \cdot 2^{o(n)}:$
$$
\Bigg(\vec  A \rand \Z_q^{n \times m},\,\, \ket{\psi_{\vec y}}=\sum_{\substack{\vec x \in \Z_q^m\\ \vec A \vec x = \vec y}}\rho_{\sigma}(\vec x) \,\ket{\vec x}, \,\,\vec y\in \Z_q^n \Bigg)\,\, \approx_c \,\,\,\, \Bigg(\vec  A \rand \Z_q^{n \times m}, \,\,\ket{\vec x_0},\,\, \vec A \cdot \vec x_0 \,\in \Z_q^n\Bigg)
$$
where $(\ket{\psi_{\vec y}},\vec y) \leftarrow \mathsf{GenGauss}(\vec A,\sigma)$ and where $\vec x_0 \sim D_{\Z_q^m,\frac{\sigma}{\sqrt{2}}}$ is a discrete Gaussian error.
\end{theorem}

Using our main theorem on certified-everlasting target-collapsing hashes in \Cref{thm:CETC-generalization}, we can now prove a stronger variant of \Cref{thm:Gauss-collapsing}. We show the following:

\begin{theorem}\label{thm:ajtai-certified-everlasting}
Let $\lambda \in \N$ be the security parameter, $n(\lambda) \in \N$, $q(\lambda) \in \N$ be a modulus, $m \geq 2n \log q$ and $\sigma \in (\sqrt{2m},q/\sqrt{2m})$. Then, the Ajtai hash function family
$\algo H = \{H_\lambda\}_{\lambda \in \N}$ with
$$
H_\lambda = \left\{ h_{\vec A}: \big\{\vec x \in \Z_q^m : \|\vec x\| \leq \sigma \sqrt{m/2}\big\} \rightarrow \Z_q^n \, \text{ s.t. } \, h_{\vec A}(\vec x) = \vec A \cdot \vec x \Mod{q}; \, \vec A \in \Z_q^{n \times m} \right\}.
$$
is certified everlasting $D_{\Z_q^m,\frac{\sigma}{\sqrt{2}}}$-target-collapsing assuming the quantum hardness of $\SIS_{n,q,\sigma\sqrt{2m}}^m$ and $\mathsf{LWE}_{n,q,\alpha q}^m$, for any noise ratio $\alpha \in (0,1)$ with relative noise magnitude $1/\alpha= \sigma \cdot 2^{o(n)}$.
\end{theorem}
\begin{proof}
By the Gaussian-collapsing property in \Cref{thm:Gauss-collapsing}, it follows that $\algo H$ is $D_{\Z_q^m,\frac{\sigma}{\sqrt{2}}}$-target-collapsing assuming the quantum hardness of $\mathsf{LWE}_{n,q,\alpha q}^m$, for any noise ratio $\alpha \in (0,1)$ with relative noise magnitude $1/\alpha= \sigma \cdot 2^{o(n)}$. Moreover, from the quantum hardness of $\SIS_{n,q,\sigma\sqrt{2m}}^m$ it follows that $\algo H$ is $D_{\Z_q^m,\frac{\sigma}{\sqrt{2}}}$-target-collision-resistant. Therefore, the claim follows from \Cref{thm:CETC-generalization}.
\end{proof}

As a corollary, we immediately recover the so-called strong Gaussian-collapsing property of the Ajtai hash function which was previously stated as a conjecture by Poremba~\cite{Poremba22}.

\begin{corollary}[Strong Gaussian-collapsing property]\label{SGC}\ \\
Let $\lambda \in \N$ be the security parameter, $n(\lambda) \in \N$, $q(\lambda) \in \N$ be a modulus and $m > 2n \log q$. Let $\sigma = \Omega(\sqrt{m})$ be a parameter. Then, the Ajtai hash function satisfies the strong Gaussian-collapsing property assuming the quantum hardness of $\SIS_{n,q,\sigma\sqrt{2m}}^m$ and $\mathsf{LWE}_{n,q,\alpha q}^m$, for any noise ratio $\alpha \in (0,1)$ with relative noise magnitude $1/\alpha= \sigma \cdot 2^{o(n)}$. In other words, for every $\QPT$ adversary $\algo A$,
$$
\mathsf{StrongGaussCollapseExpt}_{\algo A,n,m,q,\sigma}(0) \,\approx_c \, \mathsf{StrongGaussCollapseExpt}_{\algo A,n,m,q,\sigma}(1),
$$
where $\mathsf{StrongGaussCollapseExpt}_{\algo A,n,m,q,\sigma}(B)$ is the experiment from \Cref{fig:SGC}.
\end{corollary}
\begin{proof} 
To prove the statement, we can simply reduce the certified everlasting $D_{\Z_q^m,\frac{\sigma}{\sqrt{2}}}$-target-collapsing security of the Ajtai hash $\vec A = [\bar{\vec A} \, \| \, \bar{\vec A} \cdot \bar{\vec x} \Mod{q}] \in \Z_q^{n \times m}$ with $\bar{\vec x} \rand \bit^{m-1}$ to the
strong Gaussian-collapsing security, and invoke \Cref{thm:ajtai-certified-everlasting}. Here we rely on the fact that the distribution of $\vec A$ is statistically close to uniform by the leftover hash lemma whenever $m > 2n \log q$.
Recall that the adversary $\algo A = (\algo A_0,\algo A_1)$ in the certified-everlasting target-collapsing security experiment in \Cref{def:ev-target-collapsing} consists of a polynomially bounded algorithm $\algo A_0$ and an unbounded algorithm $\algo A_1$. Therefore, during the reduction, $\algo A_1$ can simply brute-force search for a trapdoor solution $\vec t = (\vec x,-1) \in \Z^{m}$ with $\vec x \in \bit^{m-1}$ such that $\bar{\vec A} \vec x = \bar{\vec A} \bar{\vec x} \Mod{q}$ given $\vec A \in \Z_q^{n \times m}$ as input. Note that such a vector exists because of how the matrix $\vec A$ is constructed in the experiment.
\end{proof}


\subsection{Dual-Regev Public-Key Encryption with Publicly-Verifiable Deletion}

We now consider the following Dual-Regev encryption scheme introduced by Poremba~\cite{Poremba22}.

\begin{construction}[Dual-Regev $\mathsf{PKE}$ with Publicly-Verifiable Deletion]\label{cons:dual-regev-cd}
Let $n \in \N$ be the security parameter, $m \in \N$ and $q$ be a prime. Let $\alpha \in (0,1)$ and $\sigma = 1/\alpha$ be parameters.
The Dual-Regev $\mathsf{PKE}$ scheme $\mathsf{DualPKECD} = (\KeyGen,\Enc,\Dec,\Del,\Vrfy)$ with certified deletion is defined as follows:
\begin{description}
\item $\KeyGen(1^\lambda) \rightarrow (\pk,\sk):$ sample a random matrix $\bar{\vec A} \rand \Z_q^{n\times m}$ and a vector $\bar{\vec x} \rand \bit^{m}$
and choose $\vec A = [\bar{\vec A} \| \bar{\vec A} \cdot \bar{\vec x} \Mod{q}]$.
Output $(\pk,\sk)$, where $\pk=\vec A \in \Z_q^{n \times (m+1)}$ and $\sk = (-\bar{\vec x}, 1) \in \Z_q^{m+1}$.
\item $\Enc(\pk,b) \rightarrow (\vk,\ket{\ct})$: parse the public key as $\vec A \leftarrow \pk$. To encrypt a single bit $b \in \bit$, generate the following pair for a random $\vec y \in \Z_q^n$:
$$
\vk \leftarrow (\vec A, \vec y), \quad \ket{\ct} \leftarrow \sum_{\vec s \in \Z_q^n} \sum_{\vec e \in \Z_q^{m+1}} \rho_{q/\sigma}(\vec e) \, \omega_q^{-\langle\vec s,\vec y \rangle}\ket{\vec s^\intercal \vec A + \vec e^\intercal +b \cdot (0,\dots,0, \lfloor\frac{q}{2} \rfloor)},
$$
where $\vk$ is the public verification key and $\ket{\ct}$ is an $(m+1)$-qudit quantum ciphertext.


\item $\Dec(\sk,\ket{\ct}) \rightarrow \bit:$ to decrypt, measure $\ket{\ct}$ in the computational basis with outcome $\vec c \in \Z_q^m$. Compute $\vec c^\intercal \cdot \sk \in \Z_q$ and output $0$, if it is closer to $0$ than to $\lfloor\frac{q}{2}\rfloor$, and output $1$, otherwise.

\item $\Del(\ket{\ct}) \rightarrow \pi:$ Measure $\ket{\ct}$ in the Fourier basis and output the measurement outcome $\pi \in \Z_q^{m+1}$.
\item $\Vrfy(\vk,\pi) \rightarrow \{\top,\bot\}:$ to verify a deletion certificate $\pi \in \Z_q^{m+1}$, parse $(\vec A,\vec y) \leftarrow \vk$ and output $\top$, if $\vec A \cdot \pi = \vec y \Mod{q}$ and $\| \pi \| \leq \sqrt{m+1}/\sqrt{2}\alpha$, and output $\bot$, otherwise.
\end{description}
\end{construction}


%%
Let us now illustrate how the deletion procedure takes place. Recall from \Cref{lem:duality} that the Fourier transform of the ciphertext $\ket{\ct}$ results in the \emph{dual} quantum state
\begin{align}\label{eq:dual-with-phase}
\ket{\widehat{\ct}}=\sum_{\substack{\vec x \in \Z_q^{m+1}:\\ \vec A \vec x = \vec y \Mod{q}}}\rho_{\sigma}(\vec x) \, \omega_q^{\langle\vec x,b \cdot (0,\dots,0,  \lfloor\frac{q}{2} \rfloor)\rangle} \,\ket{\vec x}.
\end{align}
In other words, a Fourier basis measurement of $\ket{\ct}$ necessarily erases all information about the plaintext $b \in \bit$ and results in a \emph{short} vector $\pi \in \Z_q^{m+1}$ such that $\vec A \cdot \pi = \vec y \Mod{q}$. Hence, to publicly verify a deletion certificate we can simply check whether it is a solution to the $\ISIS$ problem specified by the verification key $\vk=(\vec A,\vec y)$. Using \Cref{thm:ajtai-certified-everlasting}, we obtain the following:

\begin{theorem}
Let $n\in \N$ and let $q \geq 2$ be a prime modulus such that $q=2^{o(n)}$ and $m \geq 2n \log q$. Let $\sigma \in (\sqrt{2m},q/\sqrt{2m})$ and $\alpha \in (0,1)$ be a noise ratio with $1/\alpha= 2^{o(n)} \cdot \sigma$.
Then, the Dual-Regev public-key encryption scheme in \Cref{cons:dual-regev-cd} has everlasting certified deletion security assuming the quantum (subexponential) hardness of $\mathsf{LWE}_{n,q,\alpha q}^m$ and $\SIS_{n,q,\sigma\sqrt{2m}}^m$.
\end{theorem}
\begin{proof}
The proof is identical to the template used in~\cite[Theorem 7]{Poremba22}, except that the adversary is allowed to be computationally unbounded once the deletion certificate is submitted. This is in contrast with the original proof who considered forwarding the \emph{secret key} during the security experiment. We remark that we do not invoke the strong Gaussian-collapsing property to prove the indistinguishability of the hybrids; instead we use the (stronger) notion of certified everlasting $D_{\Z_q^m,\frac{\sigma}{\sqrt{2}}}$-target-collapsing property of the Ajtai hash shown in \Cref{thm:ajtai-certified-everlasting}. This results in the stronger notion of everlasting certified
deletion security.
\end{proof}



\subsection{Dual-Regev (Leveled) Fully Homomorphic Encryption with Publicly-Verifiable Deletion}

In this section, we recall the Dual-Regev (leveled) fully homomorphic encryption scheme with publicly-verifiable deletion introduced by Poremba~\cite{Poremba22}. The scheme is based on the \emph{dual variant} of of the (leveled) $\FHE$ scheme by Gentry, Sahai and Waters~\cite{GSW2013,mahadev2018classical}.

Let $\lambda \in \N$ be the security parameter. Suppose we would like to evaluate $L$-depth circuits consisting of $\mathsf{NAND}$ gates. We choose $n(\lambda,L) \gg L$ and a prime $q=2^{o(n)}$. Then, for integer parameters $m \geq 2 n \log q$ and $N = (m+1) \cdot \lceil \log q \rceil$, we let $\vec I$ be the $(m+1) \times (m+1)$ identity matrix and let
$\vec G = [\vec I \, \| \, 2 \vec I \, \| \, \dots \, \| \, 2^{\lceil \log q \rceil -1} \vec I] \in \Z_q^{(m+1) \times N}$ denote the so-called \emph{gadget matrix} which converts a binary representation of a vector back to its original vector representation over the field $\Z_q$. 
Note that the associated (non-linear) inverse operation $\vec G^{-1}$ converts vectors in $\Z_q^{m+1}$ to their binary representation in $\bit^N$. In other words, we have that $\vec G^{-1} \cdot \vec G = \vec I$ acts as the identity.


\begin{construction}[Dual-Regev leveled $\mathsf{FHE}$ scheme with certified deletion]\label{cons:FHE-cd}
Let $\lambda \in \N$ be the security parameter.
The Dual-Regev (leveled) $\mathsf{FHE}$ scheme $\mathsf{DualFHECD} = (\KeyGen,\Enc,\Dec,\Eval,\Del,\Vrfy)$ with certified deletion consists of the following algorithms.
\begin{description}
\item $\KeyGen(1^\lambda) \rightarrow (\pk,\sk):$ sample $\bar{\vec A} \rand \Z_q^{n\times m}$ and vector $\bar{\vec x} \rand \bit^{m}$
and let $\vec A = [\bar{\vec A} \| \bar{\vec A} \cdot \bar{\vec x} \Mod{q}]^\intercal$.
Output $(\pk,\sk)$, where $\pk=\vec A \in \Z_q^{(m+1) \times n}$ and $\sk = (-\bar{\vec x}, 1) \in \Z_q^{m+1}$.
\item $\Enc(\pk,x) \rightarrow (\vk,\ket{\ct}):$ to encrypt a bit $x\in \bit$, parse the public key as $\vec A \in \Z_q^{(m+1) \times n} \leftarrow \pk$ and generate the following pair consisting of a verification key and ciphertext for a random $\vec Y \in \Z_q^{n \times N}$ with columns $\vec y_1,\dots,\vec y_N \in \Z_q^{n}$:
$$
\vk \leftarrow (\vec A,\vec Y), \quad\,\,
\ket{\ct} \leftarrow \sum_{\vec S \in \Z_q^{n \times N}} \sum_{\vec E \in \Z_q^{(m+1)\times N}} \rho_{q/\sigma}(\vec E) \, \omega_q^{-\Tr[\vec S^\intercal \vec Y]} \ket{\vec A\cdot \vec S + \vec E + x \cdot \vec G},
$$
where $\vec G \in \Z_q^{(m+1)\times N}$ denotes the \emph{gadget matrix} and where $\sigma = 1/\alpha$.

\item $\Eval(\mathsf{C}_0,\mathsf{C}_1) \rightarrow \mathsf{C}_0 \mathsf{C}_1 \mathsf{C}$: to apply a $\mathsf{NAND}$ gate onto two registers $\mathsf{C}_0$ and $\mathsf{C}_1$ (possibly part of a larger ciphertext), append an ancilla system $\ket{\vec 0}_{\mathsf{C}}$, and apply the unitary $U_{\mathsf{NAND}}$, defined by
$$
U_{\mathsf{NAND}}: \quad \ket{\vec X}_{\mathsf{C}_0} \otimes \ket{\vec Y}_{\mathsf{C}_1} \otimes \ket{\vec Z}_\mathsf{C} \quad \rightarrow \quad  \ket{\vec X}_{\mathsf{C}_0} \otimes \ket{\vec Y}_{\mathsf{C}_1} \otimes \ket{\vec Z + \vec G - \vec X \cdot \vec G^{-1}(\vec Y) \Mod{q}}_{\mathsf{C}},
$$
where $\vec X,\vec Y,\vec Z \in \Z_q^{(m+1)\times N}$.
Output the resulting registers $\mathsf{C}_0 \mathsf{C}_1 \mathsf{C}$.


\item $\Dec(\sk,\mathsf{C}) \rightarrow \bit \, \mathbf{or} \, \bot:$ measure the register $\mathsf{C}$ in the computational basis to obtain an outcome $\vec C \in \Z_q^{(m+1)\times N}$ and compute $c = \sk^\intercal \cdot \vec c_N \in \Z \cap (-\frac{q}{2},\frac{q}{2}]$, where $\vec c_N \in \Z_q^{m+1}$ is the $N$-th column of $\vec C$; output $0$, if $c$
is closer to $0$ than to $\lfloor\frac{q}{2}\rfloor$,
and output $1$, otherwise.

\item $\Del(\ket{\ct}) \rightarrow \pi:$ measure $\ket{\ct}$ in the Fourier basis with outcomes $\pi = (\pi_1|\dots|\pi_N) \in \Z_q^{(m+1)\times N}$.

\item $\Vrfy(\vk,\pk,\pi) \rightarrow \bit:$ to verify the deletion certificate $\pi = (\pi_1\|\dots\|\pi_N) \in \Z_q^{(m+1)\times N}$, parse $(\vec A \in \Z_q^{(m+1) \times n},(\vec y_1 \|\dots \|\vec y_N)  \in \Z_q^{n \times N}) \leftarrow \vk$ and output $\top$, if both $\vec A^\intercal \cdot \pi_i = \vec y_i \Mod{q}$ and $\| \pi_i \| \leq \sqrt{m+1}/\sqrt{2}\alpha$ for every $i \in [N]$, and output $\bot$, otherwise.
\end{description}
\end{construction}

For additional details on the correctness of the scheme, we refer to Section $9$ of \cite{Poremba22}.

\begin{theorem}\label{thm:FHE-CD-security} Let $L$ be an upper bound on the $\mathsf{NAND}$-depth of the circuit which is to be evaluated. Let $n\in \N$ and $q$ be a prime modulus with $n=n(\lambda,L) \gg L$, $q=2^{o(n)}$ and $m \geq 2n \log q$, each parameterized by $\lambda \in \N$. Let $N = (m+1) \cdot \lceil \log q \rceil$ be an integer. Let $\sigma \in (\sqrt{2m},q/\sqrt{2m})$ and let $\alpha \in (0,1)$ such that $1/\alpha= 2^{o(n)} \cdot \sigma$.
Then, $\mathsf{DualFHECD}$ in \Cref{cons:FHE-cd} has everlasting certified deletion security assuming the quantum (subexponential) hardness of $\SIS_{n,q,\sigma\sqrt{2m}}^m$ and $\mathsf{LWE}_{n,q,\alpha q}^m$.
\end{theorem}
\begin{proof}
The proof is identical to the template in~\cite[Theorem 10]{Poremba22}, except that the adversary is allowed to be computationally unbounded once the deletion certificate is submitted. This is in contrast with the original proof who considered forwarding the \emph{secret key} during the security experiment. We remark that we do not invoke the strong Gaussian-collapsing property to prove the indistinguishability of the hybrids; instead we use the (stronger) notion of certified everlasting $D_{\Z_q^m,\frac{\sigma}{\sqrt{2}}}$-target-collapsing property of the Ajtai hash function shown in \Cref{thm:ajtai-certified-everlasting}. This results in the stronger notion of everlasting certified
deletion security.
\end{proof}

==> generalization.tex <==
\section{General theorem}

\james{I'm sure notation below could be made more elegant}

Let $\{\cX_\secp\}_{\secp \in \bbN}, \{\cY_\secp\}_{\secp \in \bbN}$ be families of finite sets, $\{H_\secp = \{h : \cX_\secp \to \cY_\secp\}\}_{\secp \in \bbN}$ be a family of hash functions, $\{f_{\secp,0},f_{\secp,1} : \cX_\secp \to \{e^{i \theta} : \theta \in [0,2\pi]\}\}_{\secp \in \bbN}$ be two families of phase functions, $\{D_\secp: \cX_\secp \to [0,1]\}_{\secp \in \bbN}$ be a family of distributions, and $\{M_{\secp,h}\}_{\secp \in \bbN, h \in H_\secp}$ be a family of projective measurements in the $\{\cX_\secp\}_{\secp \in \bbN}$-basis. We will now drop the indexing by $\secp$ for convenience. 

For $h \in H$, define \[\ket{\psi_{h,0}}_{X,Y} \coloneqq \sum_{x \in \cX} f_0(x)\sqrt{D(x)}\ket{x}_X\ket{h(x)}_Y, ~~ \ket{\psi_{h,1}}_{X,Y} \coloneqq \sum_{x \in \cX} f_1(x)\sqrt{D(x)}\ket{x}_X\ket{h(x)}_Y,\] and for $h \in H, y \in \cY$, define the following normalized states \[\ket{\psi_{h,y,0}}_X \propto \sum_{x \in \cX : h(x)=y} f_0(x)\sqrt{D(x)}\ket{x}_X, ~~ \ket{\psi_{h,y,1}}_X \propto \sum_{x \in \cX: h(x) = y} f_1(x)\sqrt{D(x)}\ket{x}_X.\] Then, for $h \in H, y \in \cY, b \in \{0,1\}$, let \[\left\{\ket{\psi^m_{h,y,b}}_X\right\}_m\] be the set of possible states that result from applying measurement $M_h$ to $\ket{\psi_{h,y,b}}$, indexed by measurement outcomes $m$.

Now, we require three properties from the hash function $H$.

\begin{itemize}
    \item \textbf{$(f_0,f_1,M)$-phase hiding.} For all $h,y,b$, and $m$, $f_b(\cdot)$ is constant on $x \in \mathsf{Sup}(\ket{\psi_{h,y,b}^m})$.
    \item \textbf{$(D,M)$-targeted collapsing.} For $b \in \{0,1\}$, let \[\sigma_b \coloneqq \E_{h,y}\left[(h,y,\ket{\psi_{h,y,b}})\right], ~~ \widehat{\sigma}_b \coloneqq \E_{h,y,m}\left[(h,y,\ket{\psi_{h,y,b}^m})\right],\] where the first expectation is over the sampling of $h \gets H$ and measuring register $Y$ in the $\cY$-basis to obtain $y$, and the second expectation is additionally over measuring register $X$ with $M_h$. Then for any QPT adversary $\{\cA_\secp\}_{\secp \in \bbN}$ and any $b \in \{0,1\}$, \[\left|\Pr\left[\cA_\secp(\sigma_b) \to 1\right] - \Pr\left[\cA_\secp(\widehat{\sigma}_b) \to 1\right]\right| = \negl(\secp).\]
    \item \textbf{$(D,M)$-second preimage resistance.} For any QPT adversary $\{\cA_\secp\}_{\secp \in \bbN}$ and any $b \in \{0,1\}$,
    \[\Pr_{\cA_\secp\left(h,y,\ket{\psi^m_{h,y,b}}\right) \to x'}\left[x' \notin \mathsf{Sup}\left(\ket{\psi_{h,y,b}^m}\right) \wedge h(x') = y \right] = \negl(\secp),\] where the probability is additionally over the sampling of $h \gets H$, measuring register $Y$ in the $\cY$-basis to obtain $y$, and measuring register $X$ with $M_h$ to obtain left-over state $\ket{\psi_{h,y,b}^m}$.
\end{itemize}

Finally, consider the following experiment $\Exp_{H,f_0,f_1,D,M,\cA}(b)$.

\begin{enumerate}
    \item The challenger samples $h \gets H$, prepares $\ket{\psi_{h,b}}_{X,Y}$, and measures $Y$ in the $\cY$-basis to obtain $y$ and left-over state $\ket{\psi_{h,y,b}}_X$.
    \item The challenger sends $h,y,\ket{\psi_{h,y,b}}$ to $\cA$, who outputs a classical deletion certificate $\pi$ and a left-over quantum state $\rho$.
    \item If $h(\pi) = y$, output $\rho$, and otherwise output $\bot$.
\end{enumerate}

\begin{theorem}
If $H$ satisfies the above three properties with respect to $(f_0,f_1,D,M)$, then for any QPT $\{\cA_\secp\}_{\secp \in \bbN}$, \[\TD\left(\Exp_{H,f_0,f_1,D,M,\cA}(0),\Exp_{H,f_0,f_1,D,M,\cA}(1)\right) = \negl(\secp).\]
\end{theorem}



==> injOWF.tex <==
\section{Target-Collapsing from Almost Regular One-Way Functions}

\james{Putting these notes here for now. I currently don't see how to generalize this result to arbitrary or even regular OWFs, but can keep thinking about it}

\begin{itemize}
    \item Given an injective one-way function $\{f_\secp: \{0,1\}^\secp \to \{0,1\}^{\ell(\secp)}\}_\secp$ and a universal hash family $\{h_\secp : \{0,1\}^{\ell(n)} \to \{0,1\}^{\secp -1}\}_\secp$, define the function $\widehat{f}_\secp = h_\secp \circ f_\secp : \{0,1\}^n \to \{0,1\}^{n-1}$. \cite{10.5555/112331.112379} showed that this function is target collision-resistant.
    \item Since it has expected $O(1)$ number of preimages, \cite{crypto-2022-32202}'s theorem can be used to show that it is target collapsing for \emph{any} distribution.
    \item By composing with itself, we can obtain a function that is target collision-resistant and target collapsing with arbitrary compression. Thus, by our main theorem, we obtain a function that is certified everlasting targeted-collapsing.
    \item If $f_\secp$ has a trapdoor, and $h_\secp$ is efficiently invertible (we should be able to specify such an $h_\secp$), then the resulting certified everlasting target-collapsing function has a trapdoor.
\end{itemize}



\subsection{From any one-way function}


\begin{itemize}
    \item Given any compressing one-way function $\{f_\secp: \{0,1\}^\secp \to \{0,1\}^{\ell(\secp)}\}_\secp$,
    commit to bit $b$ as:
    $$ \sqrt{\frac{N_1}{N_1+N_2}} \sum_{x: f(x) = y_0} \ket{x} + (-1)^b 
    \sqrt{\frac{N_2}{N_1+N_2}}
    \sum_{x: f(x) = y_1} \ket{x}$$
    
    %and a universal hash family $\{h_\secp : \{0,1\}^{\ell(n)} \to \{0,1\}^{\secp -1}\}_\secp$, define the function $\widehat{f}_\secp = h_\secp \circ f_\secp : \{0,1\}^n \to \{0,1\}^{n-1}$. 

    
    \item Collapsing (conjecture): 
    (whenever $N_1, N_2$ are polynomially related -- not sure if we need this), the above is indistinguishable from a mixture of $\Sigma_{x: f(x) = y_0} \ket{x}$ and $\Sigma_{x: f(x) = y_1} \ket{x}$.
    This may follow from techniques in 
    \cite{crypto-2022-32202}.
    
    \item Collision-resistance:
    given $\Sigma_{x: f(x) = y_0} \ket{x}$, it is hard to find any preimage of (random) $y_1$.
    
    This should follow from the hardness of swapping (for fixed $y_0$, $y_1$), one superposition over preimages to the other. This should hold regardless of the sizes $N_1, N_2$.

    \item (Finding $b$:) for honest binding/correctness - need to parallel repeat since POVM will err with some probability.
        
    \item If $f_\secp$ has a trapdoor, then the resulting certified everlasting target-collapsing function has a trapdoor.
\end{itemize}

==> main-theorem-old.tex <==
\section{Main Theorem: Certified Everlasting Target-Collapsing}

Collapsing can be considered a quantum analogue of classical collision-resistance. In the classical setting, a weaker security notion has also been studied, called \emph{target}-collision-resistance \cite{10.1145/73007.73011}, which requires that for any \emph{fixed} input $x$, no polynomial-time adversary can find a collision $x' \neq x$ such that $h(x) = h(x')$. We now formalize this definition, and then introduce a quantum analogue which we call \emph{target-collapsing}.

\begin{definition}[Target-Collision-Resistant Hash Function] A hash function family $\algo H = \{H_\lambda\}_{\lambda \in \N}$ is target-collision-resistant if, for every $\QPT$ adversary $\algo A$,
$$
|
\Pr[ \mathsf{TargetCollRes}_{\algo H,\algo A,\lambda}=1]| \leq \negl(\lambda).
$$
Here, the experiment $\mathsf{TargetCollRes}_{\algo H,\algo A,\lambda}$ is defined as follows:

\begin{enumerate}
    \item $\algo A$ sends an input $x \in \{0,1\}^{m(\secp)}$ to the challenger.
    \item The challenger samples a random hash function $h \rand H_\secp$ and sends $h$ to $\algo A$.
    \item $\algo A$ responds with another input $x' \in \{0,1\}^{m(\secp)}$.
    \item The experiment outputs 1 if $x \neq x'$ and $h(x) = h(x')$.
\end{enumerate}

\end{definition}

\begin{definition}[Target-Collapsing Hash Function]\label{def:targeted-collapsing} A hash function family $\algo H = \{H_\lambda\}_{\lambda \in \N}$ is target-collapsing if, for every $\QPT$ adversary $\algo A$,
$$
|
\Pr[ \mathsf{TargetCollapseExp}_{\algo H,\algo A,\lambda}(0)=1] - \Pr[ \mathsf{TargetCollapseExp}_{\algo H,\algo A,\lambda}(1)=1]
| \leq \negl(\lambda).
$$
Here, the experiment $\mathsf{TargetCollapseExp}_{\algo H,\algo A,\lambda}(b)$ is defined as follows:
\begin{enumerate}

    \item $\algo A$ sends an $m(\lambda)$-qubit quantum state
    in system $X$ to the challenger.
    
    \item The challenger samples a random hash function $h \rand H_\lambda$
    and coherently computes $h$ (into an auxiliary system $Y$) given the state in system $X$. The challenger then measures system $Y$ in the computational basis, which results in an outcome $y \in \bit^{n(\lambda)}$.
\item If $b=0$, the challenger does nothing. Else, if $b=1$, the challenger additionally measures system $X$ in the computational basis. Finally, the challenger sends the outcome state in systems $X$ to $\algo A$, together with the string $y \in \bit^{n(\lambda)}$ and a classical description of $h$.

\item $\algo A$ returns a bit $b'$, which we define as the output of the experiment.
\end{enumerate}
\end{definition}



\begin{definition}[Certified Everlasting Target-Collapsing] A hash family $\algo H = \{H_\lambda\}_{\lambda \in \N}$ is certified everlasting target-collapsing if, for any
$\algo A = (\algo A_0,\algo A_1)$ consisting of a computationally bounded algorithm $\algo A_0$ and a computationally unbounded algorithm $\algo A_1$, it holds that
$$
|
\Pr[ \mathsf{EvTargetCollapseExp}_{\algo H,\algo A,\lambda}(0)=1] - \Pr[ \mathsf{EvTargetCollapseExp}_{\algo H,\algo A,\lambda}(1)=1]
| \leq \negl(\lambda).
$$
Here, the experiment $\mathsf{EvTargetCollapseExp}_{\algo H,\algo A,\lambda}(b)$ is defined as follows:
\begin{enumerate}
   \item The adversary sends an $m(\lambda)$-qubit quantum state
    in system $X$ to the challenger.
    
    \item The challenger samples a random hash function $h \rand H_\lambda$
    and coherently computes $h$ (into an auxiliary system $Y$) given the state in system $X$. The challenger then measures system $Y$ in the computational basis, which results in an outcome $y \in \bit^{n(\lambda)}$.
\item If $b=0$, the challenger does nothing. Else, if $b=1$, the challenger additionally measures system $X$ in the computational basis. Finally, the challenger sends the outcome state in system $X$ to $\algo A$, together with the string $y \in \bit^{n(\lambda)}$ and a classical description of $h$.

\item $\algo A_0$ sends a classical certificate $\pi \in \bit^{m(\lambda)}$ to the challenger, and 
then forwards a polynomial-sized quantum state to $\algo A_1$.

\item The challenger checks if $h(\pi)=y$. If true, the challenger replies with $\top$ and the game continues; else, the challenger outputs $\bot$ and $\algo A$ loses.

\item $\algo A_1$ returns a bit $b'$, which we define as the output of the experiment.
\end{enumerate}
\end{definition}


%\section{Target-Collapsing Hashes and their Applications}

%\james{we should probably combine sections 4 and 5 into one section titled Certified Everlasting Target-Collapsing}

Our main theorem is the following: 

\begin{theorem}\label{thm:targeted-collapsing-CD} 

Let $\algo H = \{H_\lambda\}_{\lambda \in \N}$ be a hash function family which is both target-collapsing and target-collision-resistant. Then, $\algo H$ is certified everlasting target-collapsing, i.e. for any adversary
$\algo A = (\algo A_0,\algo A_1)$, where $\algo A_0$ is computationally bounded and $\algo A_1$ is computationally unbounded,
$$
|\Pr[\mathsf{EvTargetCollapseExp}_{\algo H,\algo A,\lambda}(0)] - \Pr[\mathsf{EvTargetCollapseExp}_{\algo H,\algo A,\lambda}(1)]| \leq \negl(\lambda). 
$$
\end{theorem}

%\subsection{Proof of certified everlasting collapsing}

%To prove \Cref{thm:targeted-collapsing-CD}, 


\begin{proof}

We consider the following hybrids. 

\begin{itemize}
    \item $\mathsf{Exp}_0(b)$:
\begin{enumerate}
   \item The adversary sends an $m(\lambda)$-qubit quantum state $\rho$ in a system $X$ to the challenger.
    
    \item The challenger samples a random hash function $h \rand H_\lambda$
    and coherently computes $h$ into an auxiliary system $Y$ initialized to $\ket{0^n}$.
    The challenger then measures $Y$ in the computational basis, which results in $y \in \bit^{n}$ and a partially measured state $\rho_y$.
\item If $b=0$, the challenger does nothing. Else, if $b=1$, the challenger additionally measures system $X$ in the computational basis. Finally, the challenger sends the outcome state in system $X$ to $\algo A$, together with the string $y \in \bit^{n(\lambda)}$ and a classical description of $h$.

\item $\algo A_0$ sends a classical certificate $\pi \in \bit^{m(\lambda)}$ to the challenger, and 
then forwards a polynomial-sized quantum state to $\algo A_1$.

\item The challenger checks if $h(\pi)=y$. If true, the challenger replies with $\top$ and the game continues; else, the challenger outputs $\bot$ and $\algo A$ loses.

\item $\algo A_1$ returns a bit $b'$, and wins if $b=b'$.
\end{enumerate}

    \item $\mathsf{Exp}_1(b)$:
    \begin{enumerate}
   \item The adversary sends an $m(\lambda)$-qubit quantum state $\rho$ in a system $X$ to the challenger.
    
    \item The challenger samples a random hash function $h \rand H_\lambda$
    and coherently computes $h$ into an auxiliary system $Y$ initialized to $\ket{0^n}$.
    The challenger then measures $Y$ in the computational basis, which results in $y \in \bit^{n}$ and a partially measured state $\rho_y$.
    
        \item The challenger samples a random string, $z \rand \bit^m$, prepares a $\ket{+}$ state in system $C$ and applies a controlled-$\mathsf{Z}^{z}$ operation, resulting in the state $\sigma$ given by
$$
\sigma_{CX} = \frac{1}{2} \sum_{c,c' \in \bit} \ketbra{c}{c'}_C \otimes \mathsf{Z}^{c \cdot z}{\rho_y}_X \left(\mathsf{Z}^{c' \cdot z}\right)^\dag.
$$
and sends system $X$ to $\algo A_0$, together with $y \in \bit^n$ and a classical description of $h$.

\item $\algo A_0$ replies with a certificate $\pi \in \bit^m$, and sends a quantum state $\rho_{\aux,c}$ to $\algo A_1$.
\item 
The challenger checks if $h(\pi)=y$. If yes, the game continues; else, $\algo A$ loses. Then, the challenger measures system $C$ with outcome $c'$. If $c'=b$, the game continues; else the challenger aborts and $\algo A$ wins.
\item $\algo A_1$ sends $b' \in \bit$ to the challenger.
\item The challenger checks if $b'=b$. If true, $\algo A$ wins.
    \end{enumerate}

\item $\mathsf{Exp}_2(b)$:
    \begin{enumerate}
  \item The adversary sends an $m(\lambda)$-qubit quantum state $\rho$ in a system $X$ to the challenger.
    
    \item The challenger samples a random hash function $h \rand H_\lambda$
    and coherently computes $h$ into an auxiliary system $Y$ initialized to $\ket{0^n}$.
    The challenger then measures $Y$ in the computational basis, which results in $y \in \bit^{n}$ and a partially measured state $\rho_y$.
    
        \item The challenger samples a random string, $z \rand \bit^m$, prepares a $\ket{+}$ state in system $C$ and applies a controlled-$\mathsf{Z}^{z}$ operation, resulting in the state $\sigma$ given by
$$
\sigma_{CX} = \frac{1}{2} \sum_{c,c' \in \bit} \ketbra{c}{c'}_C \otimes \mathsf{Z}^{c \cdot z}{\rho_y}_X \left(\mathsf{Z}^{c' \cdot z}\right)^\dag.
$$
and sends system $X$ to $\algo A_0$, together with $y \in \bit^n$ and a classical description of $h$.

\item $\algo A_0$ replies with a certificate $\pi \in \bit^m$, and sends a quantum state $\rho_{\aux,c}$ to $\algo A_1$.
\item 
The challenger checks if $h(\pi)=y$. If yes, the game continues; else, $\algo A$ loses. Then, the challenger applies the following projective measurement to system $C$:
$$
\Big\{\proj{\phi_\pi^{ z}},I - \proj{\phi_\pi^{ z}}\Big\} \,\quad \text{ with } \quad
\ket{\phi_\pi^{ z}} = \frac{1}{\sqrt{2}}  ( \ket{0} +  (-1)^{\langle \pi, z \rangle } \ket{1}).
$$
If the measurement succeeds, the game continues; else the challenger aborts. Finally, the challenger measures system $C$ with outcome $c'$. If $c'=b$, the game continues; else the challenger aborts.
\item $\algo A_1$ sends $b' \in \bit$ to the challenger.
\item The challenger checks if $b'=b$. If true, $\algo A$ wins.
    \end{enumerate}

Finally, we also use the following hybrid which is convenient for the sake of the proof.

\item $\mathsf{Exp}_3(b)$:
     \begin{enumerate}
   \item The adversary sends an $m(\lambda)$-qubit quantum state $\rho$ in a system $X$ to the challenger.
    
    \item The challenger samples a random hash function $h \rand H_\lambda$
    and coherently computes $h$ into an auxiliary system $Y$ initialized to $\ket{0^n}$.
    The challenger then measures systems $XY$ in the computational basis, which results in outcomes $x_0 \in \bit^m$ and $y=h(x_0) \in \bit^{n}$.
    
        \item The challenger samples a random string, $z \rand \bit^m$, prepares a $\ket{+}$ state in system $C$ and applies a controlled-$\mathsf{Z}^{z}$ operation, resulting in the state $\sigma$ given by
$$
\sigma_{CX} = \frac{1}{2} \sum_{c,c' \in \bit} \ketbra{c}{c'}_C \otimes \mathsf{Z}^{c \cdot z}{\proj{x_0}}_X \left(\mathsf{Z}^{c' \cdot z}\right)^\dag.
$$
and sends system $X$ to $\algo A_0$, together with $y \in \bit^n$ and a classical description of $h$.

\item $\algo A_0$ replies with a certificate $\pi \in \bit^m$, and sends a quantum state $\rho_{\aux,c}$ to $\algo A_1$.
\item 
The challenger checks if $h(\pi)=y$. If yes, the game continues; else, $\algo A$ loses. Then, the challenger applies the following projective measurement to system $C$:
$$
\Big\{\proj{\phi_\pi^{ z}},I - \proj{\phi_\pi^{ z}}\Big\} \,\quad \text{ with } \quad
\ket{\phi_\pi^{ z}} = \frac{1}{\sqrt{2}}  ( \ket{0} +  (-1)^{\langle \pi, z \rangle } \ket{1}).
$$
If the measurement succeeds, the game continues; else the challenger aborts. Finally, the challenger measures system $C$ with outcome $c'$. If $c'=b$, the game continues; else the challenger aborts.
\item $\algo A_1$ sends $b' \in \bit$ to the challenger.
\item The challenger checks if $b'=b$. If true, $\algo A$ wins.
    \end{enumerate}
\end{itemize}

Before we analyze the probability of distinguishing between the consecutive hybrids, we first show that the following statements hold for the final experiment $\mathsf{Exp}_3$:

\begin{claim}\label{claim:identical-certificate}
With overwhelming probability, the certificate $\pi$ returned by the adversary in
$\mathsf{Exp}_3$ is identical to the pre-image $x_0$ obtained by the challenger. In other words,\james{something that is not explicitly captured in the statement below is the fact that the adversary may have some state from earlier that is entangled with $\sigma$}
$$
\Pr \left[
 h(\pi) = y
\,\,\, \wedge \,\,\,
\pi \,\neq\, x_0
 \,\, \vline \,\, \substack{
 z \rand \bit^m\\
(\pi, \rho_{\aux}) \leftarrow \algo A_0(\sigma_X^{z})  }\right] \leq \negl(\lambda),
$$
where $y = h(x_0) \in \bit^{n}$ is the image and where $\sigma_X^{z}$ is the reduced state %\james{Isn't the reduced state just $\ket{\vec x_0}$? If so, we wouldn't have to sample $\vec z$ in the above game, and we can just give $\cA_0$ the vector $\vec x_0$ (which directly corresponds to targeted collision-resistance)} 
with respect to
$$
\sigma_{CX} = \frac{1}{2} \sum_{c,c' \in \bit} \ketbra{c}{c'}_C \otimes \mathsf{Z}^{c \cdot z}{\proj{x_0}}_X \left(\mathsf{Z}^{c' \cdot z}\right)^\dag.
$$
\end{claim}
\begin{proof}
Suppose for the sake of contraction that the probability is at least $1/\poly(\lambda)$. We now show that we can use $\algo A_0$ to break the target-collision-resistance of the hash family $\algo H = \{H_\lambda\}_{\lambda \in \N}$. 

Our reduction proceeds as follows:
\begin{enumerate}
 \item Run $\algo A_0$ to obtain an $m(\lambda)$-qubit quantum state $\rho$ in system $X$.

\item Measure system $X$ and send the outcome $x_0$ to the challenger.
    
\item Once the challenger replies with a description of a hash function $h \rand H_\lambda$, send the register $\ket{x_0}$, the image $y = h(x_0)$ as well as a description of $h$ to $\algo A_0$.

\item When $\algo A_0$ outputs $(\pi, \rho_{\aux})$, discard $\rho_{\aux}$ and output $(x_0,\pi)$.
\end{enumerate}
Notice that the state $\ket{x_0}$ which is sent to $\algo A_0$ is identical to the reduced state $\sigma_X$ with respect to $\sigma_{CX}$.
By assumption, $\algo A_0$ outputs a valid certificate $\pi \neq x_0$ such that $h(\pi) = h(x_0)$ with probability at least $1/\poly(\lambda)$. Thus, we have broken the target-collision-resistance of $\algo H$.
\end{proof}

\begin{claim}\label{claim:measurement-succeeds-wp-1}
If the challenger accepts the deletion certificate $\pi$ in Step $5$ of $\mathsf{Exp}_3$, then 
the subsequent projective measurement performed by the challenger succeeds with overwhelming probability.
\end{claim}
\begin{proof}
This follows from \Cref{claim:identical-certificate}, which states that the certificate $\pi$ returned by the adversary in
$\mathsf{Exp}_3$ is identical to the pre-image produced by the challenger with all but negligible probability.
Therefore, the projective measurement must also succeed with overwhelming probability.
\end{proof}

We now show the following:

\begin{claim}
$$
\mathsf{Adv}(\mathsf{Exp}_2) = 0.
$$
\end{claim}
\begin{proof}
We can now directly claim that the advantage is zero as follows. First, in the case that the challenger aborts (either because the deletion certificate is invalid or their projection fails), the experiment does not involve $b$, and thus the advantage of the adversary is $0$. Second, in the case that the challenger's projection succeeds, the register $C$ is either in the state
$$
\ket{\phi_\pi^{\vec z}} = \frac{1}{\sqrt{2}}  ( \ket{0} +  (-1)^{\langle \pi, \vec z \rangle } \ket{1}) \quad\,\, \text{ or } \quad\,\, (\ket{\phi_\pi^{\vec z}})^\perp = \frac{1}{\sqrt{2}}  ( \ket{0} -  (-1)^{\langle \pi, \vec z \rangle } \ket{1}) 
$$
for some $z \in \bit^m$, and thereby completely
unentangled from system $A$. Notice that the challenger's measurement of system $C$ with outcome $c'$ results in a uniformly random bit, which completely masks $b$. Therefore, the adversary's overall advantage in $\mathsf{Exp}_2$ is identical to $0$. 
\end{proof}
Next, we argue the following:

\begin{claim}
$$
|\mathsf{Adv}(\mathsf{Exp}_2) - \mathsf{Adv}(\mathsf{Exp}_1) | \,\leq \, \negl(\lambda).
$$    
\end{claim}
\begin{proof}
Recall that \Cref{claim:measurement-succeeds-wp-1} shows that the projective measurement performed by the challenger in Step $5$ of $\mathsf{Exp}_3$ succeeds with overwhelming probability.
We now argue that the same is also true for $\mathsf{Exp}_2$. 
Suppose for the sake of contradiction that there is a non-negligible difference between the success probabilities of the measurement. 
We now show that this implies the existence of an efficient distinguisher $\algo D$ that breaks the target-collapsing property of the hash family $\algo H = \{H_\lambda\}_{\lambda \in \N}$. 

Our reduction proceeds as follows:
The distinguisher $\algo D$ runs $\algo A_0$ to obtain an $m$-qubit state $\rho$ in system $X$,
and forwards it to the challenger who responds
with a description of a hash function $h \rand H_\lambda$, an image $y \in \bit^m$ and a state $\rho_y$ in system $X$
which is either a partially measured state (consisting of a superposition of pre-images)
or a single measured pre-image $\proj{x_0}$ such that $x_0 \in \bit^m$ and $h(x_0)=y$.
Next, $\algo D$ samples a random string $z \rand \bit^m$ and runs $\algo A_0$ given as input system $X$ of the state
$$
\sigma_{CX} = \frac{1}{2} \sum_{c,c' \in \bit} \ketbra{c}{c'}_C \otimes \mathsf{Z}^{c \cdot z}{\rho_y}_X \left(\mathsf{Z}^{c' \cdot z}\right)^\dag.
$$
Once $\algo A_0$ replies with a certificate $\pi$, then $\algo D$ applies the projective measurement given by
$$
\Big\{\proj{\phi_\pi^{z}},I - \proj{\phi_\pi^{z}}\Big\} \,\quad \text{ with } \quad
\ket{\phi_\pi^{z}} = \frac{1}{\sqrt{2}}  ( \ket{0} +  (-1)^{\langle \pi, z \rangle } \ket{1}).
$$
$\algo D$ outputs $1$, if the measurement succeeds, and $0$ otherwise.
If there is a non-negligible difference in success probabilities between the case when $\rho_y$ is a superposition of pre-images, or $\rho_y = \proj{x_0}$ is a single pre-image of $y$, this immediately breaks the targeted-collapsing property of $\algo H$. Therefore, the projective measurement in Step $5$ of $\mathsf{Exp}_2$ must also succeed with overwhelming probability.

Recall that $\mathsf{Exp}_2$ is identical to $\mathsf{Exp}_1$, except that the challenger applies an additional a measurement in Step $5$. Because the measurement succeeds with overwhelming probability, the advantage of the adversary must remain the same up to a negligible amount. This proves the claim.
\end{proof}

Suppose that $\algo A = (\algo A_0, \algo A_1)$ wins at $\mathsf{Exp}_0$ with probability $\epsilon >0$. We now show the following:

\begin{claim}\label{claim:exp_0-exp_1}
$$
|\mathsf{Adv}(\mathsf{Exp}_1) - \mathsf{Adv}(\mathsf{Exp}_0) | = \frac{\epsilon}{2}.
$$    
\end{claim}
\begin{proof}
Notice that the reduced state $\sigma_X$ in $\mathsf{Exp}_1$ is an equal mixture
$$
\sigma_X = \frac{1}{2} {\rho_y} + \frac{1}{2} \,  \underset{z}{\mathbb{E}} \left[\mathsf{Z}^{z}{\rho_y} \left(\mathsf{Z}^{ z}\right)^\dag \right].
$$
From \Cref{lem:random-Z} it follows that a random Pauli-$Z$ twirl induces a measurement in the computational basis. In other words, on average over the choice of $z \in \bit^m$, we have
\begin{align*}
\underset{z}{\mathbb{E}} \left[\mathsf{Z}^{z}{\rho_y} \left(\mathsf{Z}^{ z}\right)^\dag \right] & = \sum_{x \in \bit^m} \Tr[\ketbra{x}{x} \rho_y] \,\ketbra{x}{x}
\end{align*}
Therefore, the reduced state $\sigma_X$ in $\mathsf{Exp}_1$ precisely matches the state in $\mathsf{Exp}_0$:
with probability $1/2$, $\rho_y$ corresponds to a superposition of pre-images of $y$ and, with probability $1/2$, $\rho_y$ is equal to $\proj{x_0}$, i.e. it corresponds to a single (measured) pre-image $x_0$ such that $h(x_0) = y$.

Finally, we observe that $c'$ in $\mathsf{Exp}_1$ equals $b$ with probability $\frac{1}{2}$. Letting $\Pr[\mathsf{Exp}_0=1] = \epsilon$, we get
\begin{align*}
\big|\mathsf{Adv}(\mathsf{Exp}_1) - \mathsf{Adv}(\mathsf{Exp}_0) \big|
=\big| \frac{\epsilon}{2} - \epsilon \big| = \frac{\epsilon}{2}. 
\end{align*}
\end{proof}
Putting everything together, we get that $\frac{\epsilon}{2} \leq \negl(\lambda)$, and thus
\begin{claim}
$$
\epsilon = \mathsf{Adv}(\mathsf{Exp}_0) \leq \negl(\lambda).
$$    
\end{claim}

This completes the proof.

\end{proof}

\subsection{Distributional and Partial Target-Collapsing}

We now consider two ways to relax the notion of target-collapsing. First, we consider target-collapsing with respect to a particular distribution over initial inputs. That is, rather than allowing the adversary to submit an arbitrary state on register $X$ at the beginning of the experiment, we fix a state $\sum_x \sqrt{D(x)}\ket{x}$ specified by some distribution $D$ over the domain. We also consider target-collapsing where the measurement made by the challenger (in the case $b=1$) is not necessarily a full standard basis measurement. In particular, we consider a binary outcome measurement\footnote{One can easily generalize this notion to consider measurements with arbitrarily many outcomes, although we don't need that for this work.} specified by some classical predicate $P$ on the domain (which may depend on the choice of hash function $h$). That is, instead of measuring register $X$ in the standard basis, the challenger would measure a single bit obtained by evaluating $P(\cdot)$ on register $X$. The formal definition follows.

%We also generalize the notion of a hash function family to allow for sampling $h \in H_\secp$ along with some auxiliary information $\aux$, which we denote by $(h,\aux) \gets H_\secp$. We further parameterize the definition below by some function $\cZ_\secp$ 

\begin{definition}[$(\cD,\cP)$-Target-Collapsing Hash Function]
A hash function family $\cH = \{H_\secp : \{0,1\}^{m(\secp)} \to \{0,1\}^{n(\secp)}\}_{\secp \in \bbN}$ is $(\cD,\cP)$-target-collapsing for some distribution $\cD = \{D_\secp\}_{\secp \in \bbN}$ over $\{\{0,1\}^{m(\secp)}\}_{\secp \in \bbN}$ and family of predicates $\cP = \{\{P[h] : \{0,1\}^{m(\secp)} \to \{0,1\}\}_{h \in H_\secp}\}_{\secp \in \bbN}$ if, for every QPT adversary $\cA = \{\cA_\secp\}_{\secp \in \bbN}$,
$$
|
\Pr[ \mathsf{TargetCollapseExp}_{\algo H,\algo A,\algo D,\algo P,\lambda}(0)=1] - \Pr[ \mathsf{TargetCollapseExp}_{\algo H,\algo A,\algo D,\algo P,\lambda}(1)=1]
| \leq \negl(\lambda).
$$
Here, the experiment $\mathsf{TargetCollapseExp}_{\algo H,\algo A,\algo D,\algo P,\lambda}(b)$ is defined as follows:

\begin{enumerate}

    \item The challenger prepares the state \[\sum_{x \in \{0,1\}^{m(\secp)}}\sqrt{D_\secp(x)}\ket{x}\] on register $X$, and samples a random hash function $h \rand H_\lambda$. Then, it coherently computes $h$ on $X$ (into an auxiliary $n(\secp)$-qubit system $Y$) and measures system $Y$ in the computational basis, which results in an outcome $y \in \bit^{n(\lambda)}$.
    \item If $b=0$, the challenger does nothing. Else, if $b=1$, the challenger coherently computes $P[h]$ on $X$ (into an auxiliary one-qubit system $P$) and measures system $P$ in the computational basis. Finally, the challenger sends the outcome state in system $X$ to $\algo A$, together with the string $y \in \bit^{n(\lambda)}$ and a classical description of $h$.
    \item $\algo A$ returns a bit $b'$, which we define as the output of the experiment.
\end{enumerate}

We also say that the hash function family is \emph{certified everlasting} $(\cD,\cP)$-target-collapsing if for any $\algo A = (\algo A_0,\algo A_1)$ consisting of a computationally bounded algorithm $\algo A_0$ and a computationally unbounded algorithm $\algo A_1$, it holds that
$$
|
\Pr[ \mathsf{EvTargetCollapseExp}_{\algo H,\algo A,\algo D,\algo P,\lambda}(0)=1] - \Pr[ \mathsf{EvTargetCollapseExp}_{\algo H,\algo A,\algo D,\algo P,\lambda}(1)=1]
| \leq \negl(\lambda).
$$
Here, the experiment $\mathsf{EvTargetCollapseExp}_{\algo H,\algo A,\algo D,\algo P,\lambda}(b)$ is defined as follows:

\begin{enumerate}

    \item The challenger prepares the state \[\sum_{x \in \{0,1\}^{m(\secp)}}\sqrt{D_\secp(x)}\ket{x}\] on register $X$, and samples a random hash function $h \rand H_\lambda$. Then, it coherently computes $h$ on $X$ (into an auxiliary $n(\secp)$-qubit system $Y$) and measures system $Y$ in the computational basis, which results in an outcome $y \in \bit^{n(\lambda)}$.
    \item If $b=0$, the challenger does nothing. Else, if $b=1$, the challenger coherently computes $P_h$ on $X$ (into an auxiliary one-qubit system $P$) and measures system $P$ in the computational basis. Finally, the challenger sends the outcome state in system $X$ to $\algo A_0$, together with the string $y \in \bit^{n(\lambda)}$ and a classical description of $h$.
    \item $\algo A_0$ sends a classical certificate $\pi \in \bit^{m(\lambda)}$ to the challenger, and 
    then forwards a polynomial-sized quantum state to $\algo A_1$.
    \item The challenger checks if $h(\pi)=y$. If true, the challenger replies with $\top$ and the game continues; else, the challenger outputs $\bot$ and $\algo A$ loses.
    \item $\algo A_1$ returns a bit $b'$, which we define as the output of the experiment.
    
\end{enumerate}
\end{definition}

We will also define an analogous notion of $(\cD,\cP)$-target-collision-resistance, as follows.

\begin{definition}[$(\cD,\cP)$-Target-Collision-Resistant Hash Function]
A hash function family $\cH = \{H_\secp : \{0,1\}^{m(\secp)} \to \{0,1\}^{n(\secp)}\}_{\secp \in \bbN}$ is $(\cD,\cP)$-target-collision-resistant for some distribution $\cD = \{D_\secp\}_{\secp \in \bbN}$ over $\{\{0,1\}^{m(\secp)}\}_{\secp \in \bbN}$ and family of predicates $\cP = \{\{P[h] : \{0,1\}^{m(\secp)} \to \{0,1\}\}_{h \in H_\secp}\}_{\secp \in \bbN}$ if, for every QPT adversary $\cA = \{\cA_\secp\}_{\secp \in \bbN}$,
$$
|
\Pr[ \mathsf{TargetCollRes}_{\algo H,\algo A,\algo D,\algo P,\lambda}=1]| \leq \negl(\lambda).
$$
Here, the experiment $\mathsf{TargetCollRes}_{\algo H,\algo A,\algo D,\algo P,\lambda}$ is defined as follows:
\begin{enumerate}
    \item The challenger prepares the state \[\sum_{x \in \{0,1\}^{m(\secp)}}\sqrt{D_\secp(x)}\ket{x}\] on register $X$, and samples a random hash function $h \rand H_\lambda$. Next, it coherently computes $h$ on $X$ (into an auxiliary $n(\secp)$-qubit system $Y$) and measures system $Y$ in the computational basis, which results in an outcome $y \in \bit^{n(\lambda)}$. Next, it coherently computes $P[h]$ on $X$ (into an auxiliary one-qubit system $P$) and measures system $P$ in the computational basis, which results in a bit $b$. Finally, its sends the outcome state in system $X$ to $\algo A$, together with the string $y \in \{0,1\}^{n(\secp)}$ and a classical description of $h$.
    \item $\algo A$ responds with a string $x \in \{0,1\}^{m(\secp)}$.
    \item The experiment outputs 1 if $h(x) = y$ and $P_h(x) = 1-b$.
\end{enumerate}

\end{definition}


Next, we have the following theorems.

\begin{theorem}\label{thm:CETC-generalization}
Let $\cH = \{H_\secp\}_{\secp \in \bbN}$ be a hash function family that is both $(\cD,\cP)$-target-collapsing and $(\cD,\cP)$-target-collision-resistant, for some distribution $\cD$ and family of predicates $\cP$. Then, $\cH$ is certified everlasting $(\cD,\cP)$-target-collapsing.
\end{theorem}

\begin{proof}
This follows from the proof of \cref{thm:targeted-collapsing-CD} with the following tweaks:
\begin{itemize}
    \item Each experiment will start with the challenger preparing the state \[\sum_{x \in \{0,1\}^{m(\secp)}}\sqrt{D_\secp(x)}\ket{x}_X\] rather that the adversary sending an arbitrary state on register $X$.
    \item In Step 3 of $\Exp_1(b)$ and $\Exp_2(b)$, we sample $z \gets \{0,1\}$, coherently apply $P[h](\cdot)$ from the $X$ register into a fresh register $P$, and then apply a controlled-$\mathsf{Z}^{z}$ to the new register $P$, resulting in a state
    \[\propto \frac{1}{\sqrt{2}}\sum_{c \in \{0,1\}} \ket{c}_C \otimes \sum_{x : h(x)=y}\sqrt{D(x)}(-1)^{c \cdot z \cdot P[h](x)}\ket{x}_X\ket{P[h](x)}_P.\] 
    \item In Step 2 of $\Exp_3(b)$, rather than performing a full measurement in the computational basis, we measure $P[h](\cdot)$ on register $X$ to obtain a bit $d$. In Step 3, the resulting state is
    \[\propto \frac{1}{\sqrt{2}}\sum_{c \in \{0,1\}}\ket{c}_C \otimes \sum_{x:h(x)=y,P[h](x)=d}\sqrt{D(x)}(-1)^{c \cdot z \cdot d}\ket{x}_X.\]
    \item In Step 5 of $\Exp_2(b)$ and $\Exp_3(b)$, the challenger applies the following projective measurement to system $C$: 
    \[\Big\{\proj{\phi_\pi^{ z}},I - \proj{\phi_\pi^{ z}}\Big\} \,\quad \text{ with } \quad\ket{\phi_\pi^{ z}} = \frac{1}{\sqrt{2}}  ( \ket{0} +  (-1)^{z \cdot P[h](\pi)} \ket{1}).\]
    \item We prove \cref{claim:measurement-succeeds-wp-1} analogously, by reduction to the $(\cD,\cP)$-target-collision-resistance of $\cH$.
    \item To prove \cref{claim:exp_0-exp_1}, we use the fact that a random Pauli-Z twirl on register $P$ induced a measurement of the bit $P[h](\cdot)$ in the computational basis.
\end{itemize}


%\james{Follows from the proof of \cref{thm:targeted-collapsing-CD} with a few minor tweaks}
\end{proof}

\begin{theorem}\label{thm:TC-from-TCR}
Let $\cH = \{H_\secp : \{0,1\}^{m(\secp)}\to \{0,1\}^{n(\secp)}\}_{\secp \in \bbN}$ be a hash function family that is $(\cD,\cP)$-target-collision-resistant, for some distribution $\cD$ and family of predicates $\cP$. Then, $\cH$ is $(\cD,\cP)$-target-collapsing.
\end{theorem}

\begin{proof}
We will make use of the following fact (a special case of \cite[Claim 3.5]{cryptoeprint:2022/786}).

\begin{fact}\label{fact:distinguish-map}
Let $D$ be a projector, $\Pi_0,\Pi_1$ be  orthogonal projectors, and $\ket{\psi}$ be any state such that $\ket{\psi} \in \mathsf{span}(\Pi_0 + \Pi_1)$. Then,
    \[\big\| \Pi_1D\Pi_0\ket{\psi}\big\|^2 + \big\| \Pi_0D\Pi_1\ket{\psi}\big\|^2 \geq \frac{1}{2}\left(\|D\ket{\psi}\|^2-\left(\|D\Pi_0\ket{\psi}\|^2 + \|D\Pi_1\ket{\psi}\|^2\right)\right)^2.\]
\end{fact}

Now, suppose there exists an adversary $\{\cA_\secp\}_{\secp \in \bbN}$ that breaks the $(\cD,\cP)$-target-collapsing of $\cH$. Dropping parameterization by $\secp$ for convenience, we can write such an adversary as a binary outcome projective measurement $(D,I-D)$ applied to a state received from the challenger. For any $h \in H_\secp, y \in \{0,1\}^n$, let $\ket{\psi_{h,y}}$ be the normalized state such that \[\ket{\psi_{h,y}} \propto \ket{h,y}\otimes\sum_{x \in \{0,1\}^m: h(x)=y}\sqrt{D(x)}\ket{x},\] and let \[\Pi_{0,h} \coloneqq \sum_{x \in \{0,1\}^m : P[h](x) = 0}\dyad{x}{x}, ~~ \Pi_{1,h} \coloneqq \sum_{x \in \{0,1\}^m : P[h](x) = 1}\dyad{x}{x}.\]

Then, the adversary's advantage in the $(\cD,\cP)$-target-collapsing game can be written as 

\[\E_{h,y}\left[\|D\ket{\psi_{h,y}}\|^2 - \left(\|D\Pi_{0,h}\ket{\psi_{h,y}}\|^2 + \|D\Pi_{1,h}\ket{\psi_{h,y}}\|^2
\right)\right] = \nonnegl(\secp),\] where the expectation is over the sampling of $h \gets H_\secp$ and the challenger's measurement of $y$.

Thus, by \cref{fact:distinguish-map}, it follows that

\[\E_{h,y}\left[\|\Pi_{1,h}D\Pi_{0,h}\ket{\psi_{h,y}}\|^2 + \|\Pi_{0,h}D\Pi_{1,h}\ket{\psi_{h,y}}\|^2\right] = \nonnegl(\secp).\]

This completes the proof, as this expression exactly corresponds to the adversary's probability of winning the $(\cD,\cP)$-target-collision-resistance game by applying $D$ and then measuring in the computational basis.

\end{proof}

%Combined, these theorems directly imply the following.

%\begin{corollary}
%Let $\cH = \{H_\secp\}_{\secp \in \bbN}$ be a hash function family that is $(\cD,\cP)$-target-collision-resistant, for some distribution $\cD$ and family of predicates $\cP$. Then, $\cH$ is certified everlasting $(\cD,\cP)$-target-collapsing.
%\end{corollary}


==> misc.tex <==
\section{Further Thoughts on Target-Collapsing}

\begin{itemize}
    \item \james{Construction of target-collapsing from injective OWFs}
    \item \james{Examples of target-collapsing but not target-collision-resistant functions}
    \item \james{Are there examples of target-collision-resistant but not target-collapsing functions?}
\end{itemize}
